The Role of Social Support and Influencers in Social Media Communities

How can individual agents coordinate their actions to achieve a shared objective in distributed systems? This challenge spans economic, technical, and sociological domains, each confronting scalability, heterogeneity, and conflicts between individual and collective goals. In economic markets, a common currency facilitates coordination, raising the question of whether such mechanisms can be applied in other contexts. This paper explores this idea within social media platforms, where social support (likes, shares, comments) acts as a currency that shapes content production and sharing. We investigate two key questions: (1) Can social support serve as an effective coordination tool, and (2) What role do influencers play in content creation and dissemination? Our formal analysis shows that social support can coordinate user actions similarly to money in economic markets. Influencers serve dual roles, aggregating content and acting as information proxies, guiding content producers in large markets. While imperfections in information lead to a "price of influence" and suboptimal outcomes, this price diminishes as markets grow, improving social welfare. These insights provide a framework for understanding coordination in distributed environments, with applications in both sociological systems and multi-agent AI systems.

==> commands_old.tex <==
%background
%\newcommand{\Com}{\mathcal{C}}  %community
\newcommand{\Com}{C}  %community
\newcommand{\setR}{R}
\newcommand{\setT}{\mathcal{T}} 
\newcommand{\IC}{\mathcal{I}_{\Com}}
\newcommand{\UCd}{{U^{(d)}_C}}
\newcommand{\UCs}{{U^{(s)}_C}}
\newcommand{\xs}{{x^*}}

%brackets
\newcommand{\Bbl}{\Big ( }
\newcommand{\Bbr}{\Big ) }
\newcommand{\Bsbl}{\Big [ }
\newcommand{\Bsbr}{\Big ] }
\newcommand{\Bsblr}{\Big ( }
\newcommand{\Bsbrr}{\Big ) }
\newcommand{\Bsl}{{\Big \{ }}
\newcommand{\Bsr}{{\Big \} }}
\newcommand{\cb}[1]{\{#1\}}


%model
\newcommand{\Infl}{\mbox{{\tiny infl}}}
\newcommand{\opt}{\mbox{\tiny opt}}
\newcommand{\NE}{\mbox{\tiny NE}}

\newcommand{\comSet}{C}
\newcommand{\leafSet}{\comSet}
\newcommand{\infl}{y_{\Infl}}

\newcommand{\Icen}{I_0}


%problem formulation

\newcommand{\leafProductionRate}{r_p}


\newcommand{\possibleStrategy}{\mathcal{S}}
\newcommand{\possibleStrategyBudget}{\mathcal{S}(\coreBudget,\leafBudget)}

%new set of command
\newcommand{\coreBudget}{M_{\Infl}}
\newcommand{\leafBudget}{M}


\newcommand{\alternative}[1]{r_0 B_0 e^{- \frac{\alpha}{#1}} I(#1)}
\newcommand{\firstOrderAlternative}[1]{\frac{\alpha}{#1^2}e^{ - \frac{\alpha}{#1}}C_0}

%allocation
\newcommand{\leafAllocation}[1]{\comAllocation(#1)}
\newcommand{\allAllocation}{\Omega}
\newcommand{\allAllocationNE}{\Omega_{\NE}}
\newcommand{\allAllocationInfl}{\allAllocation_{\Infl}}
\newcommand{\allAllocationInflOpt}{\allAllocation^*_{\Infl}}
\newcommand{\allAllocationWelfare}{\allAllocation_{\opt}}
\newcommand{\comAllocation}{\Lambda}
\newcommand{\contAllocation}{X}
\newcommand{\coreInteract}[1]{\mu_{\Infl}(#1)}
\newcommand{\coreInteractOpt}[1]{\mu^*_{\Infl}(#1)}
\newcommand{\coreInteractVec}{\mu_{\Infl}}
\newcommand{\coreInteractVecOpt}{\mu^*_{\Infl}}

\newcommand{\setNEInfl}{{\mathcal{S}_{\Infl}}}

%utility
\newcommand{\coreUtility}[1]{U_{\Infl}(y_{\Infl}|#1)}
%\newcommand{\leafOptUtility}[1]{U_p(#1|\coreRateVec,\leafRateVec{#1})}
\newcommand{\leafOptUtility}[1]{U_c(\leafRateVec{#1}|\coreRateVec,\contAllocation,#1)}
\newcommand{\prodOptUtility}[1]{U_p(x({#1})|\coreRateVec,\comAllocation,#1)}
%\newcommand{\leafCommUtility}[1]{U_{C,p}(#1|\coreRateVec,\leafRateVec{#1})}%\leafRateVec{#1}|#1)}
\newcommand{\leafCommUtility}[1]{U_{C,p}(\leafRateVec{#1}|\coreRateVec,#1)}
\newcommand{\leafCommUtilityC}[2]{U_{C,p}(\leafRateVec{#1}|#2,#1)}
%\newcommand{\leafCommUtilityS}[1]{U_{C,p}(#1|\coreRateVecS,\leafRateVecS{#1})}
\newcommand{\leafCommUtilityS}[1]{U_{C,p}(\leafRateVecS{#1}|\coreRateVecS,#1)}

\newcommand{\leafOptUtilityInf}[1]{U^{\Infl}_c(\leafRateVec{#1}|\coreRateVec,\contAllocation,#1)}
\newcommand{\prodOptUtilityInf}[1]{U^{\Infl}_p(x({#1})|\coreRateVec,\comAllocation,#1)}
\newcommand{\prodUtilityWelfare}[1]{U_p(\allAllocationWelfare^*(\coreBudget,\leafBudget),#1)}
\newcommand{\prodUtilityNE}[1]{U_p(\allAllocation^*(\coreBudget,\leafBudget),#1)}
\newcommand{\prodUtilityNEInfl}[1]{U_p(\allAllocationInfl^*(\coreBudget,\leafBudget),#1)}
\newcommand{\prodUtilityAllocation}[1]{U_p(\allAllocation,#1)}

\newcommand{\leafUtility}[3]{U(#1,#2|#3)}
\newcommand{\utilityBetween}[2]{u(#1|#2)}

\newcommand{\delayCoreUtility}[2]{r_p B(#1|#2) e^{ - \alpha \left ( \frac{1}{\mu_{\Infl}(#1)} + \frac{1}{\mu(\infl|#2)} \right)}  I(\mu_{\Infl}(#1))I(\mu(\infl|#2))}
\newcommand{\delayCoreUtilityStable}[2]{r_p B(#1|#2) e^{ - \alpha \left ( \frac{1}{\mu^*_\Infl(#1)} + \frac{1}{\mu^*(y_0|#2)} \right)} I(\mu^*_{\Infl}(#1))I(\mu^*(\infl|#2))}
\newcommand{\delayCoreUtilityR}[2]{r_p B(z|y) e^{ - \alpha \left ( \frac{1}{#1} + \frac{1}{#2} \right)} I(#1)I(#2)}


\newcommand{\delayUtility}[2]{r_p B(#1|#2) e^{ - \frac{\alpha}{\mu(#1|#2)}}  I(\mu(#1|#2))}
\newcommand{\delayUtilityStable}[2]{r_p B(#1|#2) e^{ - \frac{\alpha}{\mu^*(#1|#2)}}  I(\mu^*(#1|#2))}


\newcommand{\simpleCoreUtility}[2]{r_p B(#1|#2) e^{ - \alpha \left ( \frac{1}{\mu_c(#1)} + \frac{1}{\mu(y_0|#2)} \right)}}



%optimization problem
\newcommand{\leafOpt}[1]{\max_{\leafAllocation{#1}}  \leafOptUtility{#1}}
\newcommand{\optcore}[1]{OPT_{\Infl}(\coreRateVec|#1)}
\newcommand{\optperiphery}[2]{OPT_c(\leafAllocation{#2}|#1,#2)}
\newcommand{\optcontperiphery}[2]{OPT_p(x(#2)|#1,#2)}
\newcommand{\optglobal}{OPT(\muc)}
\newcommand{\coreRateVec}{\coreInteractVec}
\newcommand{\coreRateVecS}{\coreInteractVecOpt}
\newcommand{\leafRateVec}[1]{\comAllocation(#1)}
%\newcommand{\leafRateVecS}[1]{\muv^*_p(#1)}
\newcommand{\Clw}[1]{\leafSet \backslash\{#1\}}
\newcommand{\Cw}[1]{\comSet \backslash\{#1\}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\strategySpace}{S}

\newcommand{\allstrategySpace}{\possibleStrategy_0}


==> content/abstract.tex <==

\begin{abstract}
How can individual agents coordinate their actions in a distributed manner to achieve a shared objective? This question arises across various systems—economic, technical, and sociological—all of which face common challenges such as scalability, heterogeneity, and conflicting individual and collective goals. In economic markets, these challenges are mitigated by the use of a common currency, which enables participants to coordinate their actions toward efficient outcomes. This raises the question of whether similar mechanisms, such as a common currency, can be applied to other systems, including technical and sociological contexts.

In this paper, we explore this idea within the context of social media, where communities form around shared interests. We propose that social support (in the form of likes, shares, and comments) functions as a currency that coordinates the actions of users in content markets. We investigate two core questions: (1) Can social support serve as a currency that shapes the production and sharing of content, and (2) What role do influencers play in coordinating content creation and dissemination?

Through formal modeling and analysis, we demonstrate that social support can act as an efficient coordination mechanism, similar to money in economic markets. Influencers play a dual role in aggregating content and acting as proxies for information, helping content producers navigate large markets. Our findings suggest that while social support as a currency leads to efficient outcomes in ideal markets, imperfections in information introduce a "price of influence," resulting in suboptimal outcomes. However, as content markets grow, this price diminishes, and social welfare approaches optimal levels. These insights offer a framework for understanding coordination in distributed environments, with potential applications to both sociological and technical systems, including multi-agent AI systems.

\end{abstract}


